Specious Sites: Tracking the Spread and Sway of Spurious News Stories at Scale

Misinformation, propaganda, and outright lies proliferate on the web, with some narratives having dangerous real-world consequences on public health, elections, and individual safety. However, despite the impact of misinformation, the research community largely lacks automated and programmatic approaches for tracking news narratives across online platforms. In this work, utilizing daily scrapes of 1,334 unreliable news websites, the large-language model MPNet, and DP-Means clustering, we introduce a system to automatically identify and track the narratives spread within online ecosystems. Identifying 52,036 narratives on these 1,334 websites, we describe the most prevalent narratives spread in 2022 and identify the most influential websites that originate and amplify narratives. Finally, we show how our system can be utilized to detect new narratives originating from unreliable news websites and to aid fact-checkers in more quickly addressing misinformation. We release code and data at https://github.com/hanshanley/specious-sites.

==> conclusion.tex <==
%\section{Conclusion}

==> dead.tex <==
\begin{table*}
\centering
\scriptsize
%\fontsize{8.5pt}{10pt}
\selectfont
\begin{tabular}{l|l|r|r|l}
Topic &  {Keywords} & \# Articles & \#Domains & Top Domains \\ \midrule
Topic 1 & ukraine,nato,russia,kiev, putin
 &63,905 & 731 & express.co.uk (4,073), rt.com (4020), sputniknews.com (2,952) \\%\hline
Topic 2 & ukraine,kiev,donbas,russia,invasion & 56,336& 722 & express.co.uk (2175), rt.com (1986), australiannationalreview.com(1669) \\
Topic 3 & putin,russia,sanction,biden,world & 45,507 & 695 &express.co.uk (3645), rt.com (2581),sputniknews.com(1978)\\
Topic 4 & ukraine,kyiv,soldier,refugee,fled & 41021 & 668 & worldcrunch.com (3525), shorenetworknews.com (2798), en.news-front.info (2328) \\
Topic 5 & vaccine,mandate,covid19,court,employer & 40950 & 798 & theepochtimes.com (1694), australiannationalreview.com (1529),childrenshealthdefense.or (1203) \\

Topic 6 & ukraine,russia,donestk,military,lugansk & 39392 & 608 & worldcrunch.com (3346),express.co.uk (2871),rt.com (2350) \\
Topic 7 & nato,russia,war,nuclear,putin & 39122& 650 & express.co.uk(3127),rt.com (2371),sputniknews.com (1825) \\
Topic 8 & ukraine,russia,soviet,kiev,crimea & 38009& 651 & worldcrunch.com(3577),rt.com (2258),express.co.uk (1847) \\

Topic 9 & ukraine,russia,soviet,kiev,crimea & 36292& 659 & worldcrunch.com(3956),stateofthenation.co(2258),en.news-front.info (1891) \\
Topic 10 & ukraine,assistance,bill,senate,crisis & 29243& 620 & rt.com(1635),sputniknews.com(1463),express.co.uk (1441) \\
\end{tabular}
\caption{\label{tab:narratives}A select of some of the top---by number of articles---narratives/topics present within our data.} 
\vspace{-5pt}
\end{table*}


\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{figures/screenshot_200344.png}
\caption{Communities of semantically similar websites. Size is determined by weighted degree (\textit{i.e.,} how similar the website is to all the other websites in the dataset). We see three distinct communities emerge: US-focused (Purple), International (Orange), and Conspiratorial (Green).
}
\label{fig:semantic-communities}
\end{figure}

\begin{table}
\centering
\fontsize{8pt}{9pt}
\selectfont
\setlength{\tabcolsep}{4pt}
\begin{tabular}{llrrr}
%\toprule 
{Topic} & Keywords &{\# Artl.}  &{\# Paragraphs. } & {Prec.}           \\  \midrule % \hline 
zerohedge 20 & russia,putin,ukraine,war,nato &397 & 787 &  97.3\%    \\ %\hline
zerohedge 15 & fed,inflation,market,rate,bank &288 & 660 &  97.0\% \\
zerohedge 912  & gas,europe,russia,energy,eu  &223 & 428 &  99.3\% \\
zerohedge 71 & price,gas,gallon,demand,high & 153 & 282 & 98.2\% \\
zerohedge 110 &job,labor,market,survey,employment & 250 & 83 & 100\% \\
\midrule 
\end{tabular}
\caption{\label{tab:precision-test} Evaluation of the precision of our topic analysis model on 25 topics (top 10 most frequently mentioned topics and 15 random topics) derived from Russian state media website articles. }  
\vspace{-0.5cm}

\end{table}


\begin{table}
\centering
\fontsize{8pt}{9pt}
\selectfont
\setlength{\tabcolsep}{4pt}
\begin{tabular}{llrrr}
%\toprule 
{Topic} & Keywords &{\# Artl.}  &{\# Paragraphs. } & {Prec.}           \\  \midrule % \hline 
x22report.com 13 & trump,patriot,people,control,election  &678 & 686 &  99.8\%    \\ %\hline
x22report.com 20 & gold,ira,retirement,trust,protect  &279 & 558 &  100\%    \\ %\hline
x22report.com 511 & central, bank,system,patriot,economic &398 & 511 &  95.7\%    \\ 
x22report.com 14 & Q trip codes &168 & 440 &  100\%   \\ 
x22report.com 21 & election,vote,ballot,fraud,cheater &84 & 216 &  100\%   \\ %\hline

\midrule 
\end{tabular}
\caption{\label{tab:precision-test} Evaluation of the precision of our topic analysis model on 25 topics (top 10 most frequently mentioned topics and 15 random topics) derived from Russian state media website articles. }  
\vspace{-0.5cm}

\end{table}


\begin{table}
\centering
\fontsize{8pt}{9pt}
\selectfont
\setlength{\tabcolsep}{4pt}
\begin{tabular}{llrrr}
%\toprule 
{Topic} & Keywords &{\# Artl.}  &{\# Paragraphs. } & {Prec.}           \\  \midrule % \hline 
americanthinker.com 5 & biden,joe,president,democrat,administration  &542 & 1101 &  93.8\%    \\
americanthinker.com 18 & ukraine,putin,russia,war,nato  &271 & 650 &  97.5\%    \\
americanthinker.com 27 & inflation,biden,price,money,spend  &202 & 521 &  99.4\%    \\
americanthinker.com 83 & abortion,roe,right,court,state  &181 & 511 &  99.2\%    \\
americanthinker.com 12 & lefirst,liberal,america,antiliberity,conservative  &312 & 495 &  97.6\%    \\
\midrule 
\end{tabular}
\caption{\label{tab:precision-test} Evaluation of the precision of our topic analysis model on 25 topics (top 10 most frequently mentioned topics and 15 random topics) derived from Russian state media website articles. }  
\vspace{-0.5cm}

\end{table}



\begin{table}
\centering
\fontsize{8pt}{9pt}
\selectfont
\setlength{\tabcolsep}{4pt}
\begin{tabular}{llrrr}
%\toprule 
{Topic} & Keywords &{\# Artl.}  &{\# Paragraphs. } & {Prec.}           \\  \midrule % \hline 
oann.com 179 & rate,fed,hike,basis,interest  &222 & 427 &  100.0\%    \\
oann.com 36& abortion,roe,law,state,wade,court  &162 & 315 &  99.0\%    \\
oann.com 2& inflation,fed,rate,recession,market  &169 & 273 &  99.6\%    \\
oann.com 10 & biden,joe,president,administration,house  &212 & 262 &  100.0\%    \\
oann.com 107 & twitter,musk,elon,company,dorsey &83 & 214 &  100.0\%    \\
\end{tabular}
\caption{\label{tab:precision-test} Evaluation of the precision of our topic analysis model on 25 topics (top 10 most frequently mentioned topics and 15 random topics) derived from Russian state media website articles. }  
\vspace{-0.5cm}

\end{table}




\begin{table}
\centering
\fontsize{8pt}{9pt}
\selectfont
\setlength{\tabcolsep}{4pt}
\begin{tabular}{llrrr}
%\toprule 
{Topic} & Keywords &{\# Artl.}  &{\# Paragraphs. } & {Prec.}           \\  \midrule % \hline 
unz.com 14 & white,black,people,race,racism  &218 & 534 &  100.0\%    \\
unz.com 557 & nato,russia,ukraine,war,military  &191 & 501 & 98.8\%    \\
unz.com 65 & putin,russia,president,west,vladimir  &206 & 417 & 89.7\%    \\
unz.com 313 & black,crime,murder,man,police  &165 & 399 & 96.5\%    \\
unz.com 51 & russia,sanction,putin,west,economy  &117 & 314 & 93.6\%    \\

\end{tabular}
\caption{\label{tab:precision-test} Evaluation of the precision of our topic analysis model on 25 topics (top 10 most frequently mentioned topics and 15 random topics) derived from Russian state media website articles. }  
\vspace{-0.5cm}

\end{table}


\begin{table}
\centering
%\fontsize{8pt}{9pt}
\scriptsize
\selectfont
\setlength{\tabcolsep}{4pt}
\begin{tabular}{llrrr}
%\toprule 
{Topic} & Keywords &{\# Artl.}  &{\# Paragraphs. } & {Prec.}           \\  \midrule % \hline 
breitbart 944 & percent,biden,approval,rating,poll  &634 & 1522 &  99.6\%    \\
breitbart 13 & ukraine,russia, putin, war,president  &557 & 937 &  99.3\% \\
breitbart 13 & migration,america, extraction, labor,economy  &229 & 854 &  100\% \\
breitbart 13 & inflation,price, percent, biden, america  &328 & 825 &  100\% \\
breitbart 63 & abortion,roe, right, court,woman  &467 & 821 &  99.8\%  \\
\end{tabular}
\caption{\label{tab:precision-test} Evaluation of the precision of our topic analysis model on 25 topics (top 10 most frequently mentioned topics and 15 random topics) derived from Russian state media website articles. }  
\vspace{-0.5cm}

\end{table}


\begin{table}
\centering
%\fontsize{8pt}{9pt}
\scriptsize
\selectfont
\setlength{\tabcolsep}{4pt}
\begin{tabular}{llrrr}
%\toprule 
{Topic} & Keywords &{\# Artl.}  &{\# Paragraphs. } & {Prec.}           \\  \midrule % \hline 
benjaminfulford.net 16 &ukraine, russia, source, polish, war  &27 & 49 &  97.8\%    \\
benjaminfulford.net 9 & coporation,biden, fake, money,regime  &26 & 45 &  100.0\% \\
benjaminfulford.net 0 & mafia,khazarian, satanist,kill, society  &22 & 33 &  100\% \\
benjaminfulford.net 13 & vaccine,virus, government, covid, fake&17 & 32 &  100\% \\
benjaminfulford.net 63 & alien,group, illuminati, plot, asian  &5 & 30 &  100.0\%  \\
\end{tabular}
\caption{\label{tab:precision-test} Evaluation of the precision of our topic analysis model on 25 topics (top 10 most frequently mentioned topics and 15 random topics) derived from Russian state media website articles. }  
\vspace{-0.5cm}

\end{table}




\begin{table}
\centering
%\fontsize{8pt}{9pt}
\scriptsize
\selectfont
\setlength{\tabcolsep}{4pt}
\begin{tabular}{llrrr}
%\toprule 
{Topic} & Keywords &{\# Artl.}  &{\# Paragraphs. } & {Prec.}           \\  \midrule % \hline 
rt.com 14 &kiev,ukraine,offensive,unprovoked, military  &1782 & 2383 &  99.8\%    \\
rt.com 1941 &minsk,ukraine,agreement,lugansk, donetsk  &1189 & 1483 &  99.0\%    \\
rt.com 141 &sanction,moscow,ukraine, eu,impose  &849 & 1341 &  99.5\%    \\
rt.com 141 &taiwan,china,beijing, island,military  &250 & 790 &  98.7\%    \\
rt.com 141 &gas,russia,eu, energy,supply  &498 & 824 &  99.3\%    \\
\end{tabular}
\caption{\label{tab:precision-test} Evaluation of the precision of our topic analysis model on 25 topics (top 10 most frequently mentioned topics and 15 random topics) derived from Russian state media website articles. }  
\vspace{-0.5cm}

\end{table}



\begin{table*}
\centering
%\fontsize{8pt}{9pt}
\scriptsize
\selectfont
\setlength{\tabcolsep}{4pt}
\begin{tabular}{llrrr}
%\toprule 
{Topic} & Keywords &{\# Artl.}  &{\# Paragraphs. } & {Prec.}           \\  \midrule % \hline 
theconservativetreehouse.com 10 &intelligence,branch,apparatus,government, surveillance  &180 & 1320 &  99.6\%    \\
theconservativetreehouse.com 10 &ukraine,russia,putin,nato,conflict &381 & 775 & 98.2\%    \\
theconservativetreehouse.com 10 &ukraine,western,military,propaganda,narrative &365 & 743 & 94.5\%    \\
theconservativetreehouse.com 10 &desantis,ron,governor,florida,trump &194 & 629 & 100.0\%    \\
theconservativetreehouse.com 10 &trump,president,document,declassify,doj &194 & 629 & 100.0\%    \\
theconservativetreehouse.com 10 &energy, oil,policy,climate,change &315 & 490 & 98.4\%    \\

\end{tabular}
\caption{\label{tab:precision-test} Evaluation of the precision of our topic analysis model on 25 topics (top 10 most frequently mentioned topics and 15 random topics) derived from Russian state media website articles. }  
\vspace{-0.5cm}

\end{table*}


\begin{table}
\centering
%\fontsize{8pt}{9pt}
\scriptsize
\selectfont
\setlength{\tabcolsep}{4pt}
\begin{tabular}{llrrr}
%\toprule 
{Topic} & Keywords &{\# Artl.}  &{\# Paragraphs. } & {Prec.}           \\  \midrule % \hline 
theconservativetreehouse.com 10 &intelligence,branch,apparatus,government, surveillance  &180 & 1320 &  99.6\%    \\
theconservativetreehouse.com 10 &ukraine,russia,putin,nato,conflict &381 & 775 & 98.2\%    \\
theconservativetreehouse.com 10 &ukraine,western,military,propaganda,narrative &365 & 743 & 94.5\%    \\
theconservativetreehouse.com 10 &desantis,ron,governor,florida,trump &194 & 629 & 100.0\%    \\
theconservativetreehouse.com 10 &trump,president,document,declassify,doj &194 & 629 & 100.0\%    \\
theconservativetreehouse.com 10 &energy, oil,policy,climate,change &315 & 490 & 98.4\%    \\

\end{tabular}
\caption{\label{tab:precision-test} Evaluation of the precision of our topic analysis model on 25 topics (top 10 most frequently mentioned topics and 15 random topics) derived from Russian state media website articles. }  
\vspace{-0.5cm}

\end{table}


\begin{table}
\centering
%\fontsize{8pt}{9pt}
\scriptsize
\selectfont
\setlength{\tabcolsep}{4pt}
\begin{tabular}{llrrr}
%\toprule 
{Topic} & Keywords &{\# Artl.}  &{\# Paragraphs. } & {Prec.}           \\  \midrule % \hline 
globalresearch.ca 5 & vaccine, covid, death, data, child &506 & 1428 &  99.6\%    \\
globalresearch.ca 5 & russia,nato,war,military,ukraine &617 & 1300 &  92.5\%    \\
globalresearch.ca 5 & ukraine,weapon,billion,aid,missile &283 & 638 &  98.1\%    \\
globalresearch.ca 5 & ukraine,nazi,asov,battalion,government &223 & 612 & 96.1\%    \\
globalresearch.ca 5 & gmo,crop,food,genetic,seed &48 & 228 & 99.5\%    \\

\end{tabular}
\caption{\label{tab:precision-test} Evaluation of the precision of our topic analysis model on 25 topics (top 10 most frequently mentioned topics and 15 random topics) derived from Russian state media website articles. }  
\vspace{-0.5cm}

\end{table}

\begin{table}
\centering
%\fontsize{9pt}{10.5pt}
\scriptsize

\setlength{\tabcolsep}{5pt}
\begin{tabular}{llrr}
Domain & CrUX rank  & Avg \# Articles  & Cohen's D \\ 
& &  Origin Topics  &   Effect Size\\ \midrule
dailymail.co.uk &  &1.063400576368876  &00.2753555814077257\\%\hline 
express.co.uk &  &0.7021505376344086&0.1504\\%\hline 

Avg & & 0.21288
\end{tabular}
\caption{\label{tab:real-originating} Most effective large popular websites in getting narratives spread onto other wesbites. Rank $<$ 1000 }  
\vspace{-5pt}
\end{table}


\begin{table}
\centering
%\fontsize{9pt}{10.5pt}
\scriptsize

\setlength{\tabcolsep}{5pt}
\begin{tabular}{lrr}
Domain & Avg \# External Articles  & Cohen's D \\ 
& per Origin Topic  &   Effect Size\\ \midrule
breitbart.com &1.619 &0.4035 \\
nypost.com &1.586 & 0.3259 \\
zerohedge.com &1.4535 &  0.209 \\
rt.com &1.559 & 0.1923\\
mirror.co.uk & 0.21 & 0.009 \\
Avg & & 0.149037100808556\\
\end{tabular}
\caption{\label{tab:real-originating} Most effective large popular websites in getting narratives spread onto other wesbites. Rank $<$ 1000 }  
\vspace{-5pt}
\end{table}

\begin{table}
\centering
%\fontsize{9pt}{10.5pt}
\scriptsize

\setlength{\tabcolsep}{5pt}
\begin{tabular}{lrr}
Domain & Avg \# Articles  & Cohen's D \\ 
& Origin Topics  &   Effect Size\\ \midrule
newsmax.com & 1.4141 & 0.37005 \\
thegatewaypundit.com &1.626 & 0.335\\
rawstory.com &0.997  & 0.1677 \\
gotquestions.org &1.160 &  0.11835 \\
bleacherreport.com &0.34 & 0.0430 \\
Avg &  &0.1114251671361563\\


\end{tabular}
\caption{\label{tab:real-originating} Most effective large popular websites in getting narratives spread onto other wesbites. Rank $<$ 1000 }  
\vspace{-5pt}
\end{table}






\begin{table}
\centering
%\fontsize{9pt}{10.5pt}
\scriptsize

\setlength{\tabcolsep}{5pt}
\begin{tabular}{lrr}
Domain & Avg \# Articles  & Cohen's D \\ 
& Origin Topics  &   Effect Size\\ \midrule
dailycaller.com & 1.752 & 0.4311 \\
banned.video & 1.5 &0.3859\\
dailywire.com &  2.093&  0.33437 \\
theepochtimes.com &1.374 &  0.28305 \\
theblaze.com & 1.412&  0.27226 \\
Avg & & 0.05588719648016633 \\

\end{tabular}
\caption{\label{tab:real-originating} Most effective large popular websites in getting narratives spread onto other wesbites. Rank $<$ 1000 }  
\vspace{-5pt}
\end{table}


\begin{table}
\centering
%\fontsize{9pt}{10.5pt}
\scriptsize
\setlength{\tabcolsep}{5pt}
\begin{tabular}{lrr}
Domain & Avg \# Articles  & Cohen's D \\ 
& Origin Topics  &   Effect Size\\ \midrule
resistthemainstream.org& 1.029 &0.3464 \\
dennismichaellynch.com & 1.345&0.342246\\
wnd.com & 0.825 &  0.32769 \\
justthenews.com & 1.609&   0.3273 \\
thelibertydaily.com &1.021 & 0.32215 \\
Avg & & 0.06537950338603808 \\

\end{tabular}
\caption{\label{tab:real-originating} Most effective large popular websites in getting narratives spread onto other wesbites. Rank $<$ 1000 }  
\vspace{-5pt}
\end{table}

\begin{table}
\centering
%\fontsize{9pt}{10.5pt}
\scriptsize
\setlength{\tabcolsep}{5pt}
\begin{tabular}{lrr}
Domain & Avg \# Articles  & Cohen's D \\ 
& Origin Topics  &   Effect Size\\ \midrule
weaselzippers.us&  2.761& 0.582993 \\
judicialwatch.org &1.2236 &0.57428965\\
populistpress.com & 1.5428 &  0.52544 \\
hannity.com & 1.4186&  0.46417665 \\
vigilantcitizen.com & 0.973684&  0.44007 \\
Avg & & 0.058735768324504785 \\

\end{tabular}
\caption{\label{tab:real-originating} Most effective large popular websites in getting narratives spread onto other wesbites. Rank $<$ 1000 }  
\vspace{-5pt}
\end{table}



\begin{table}
\centering
%\fontsize{9pt}{10.5pt}
\scriptsize
\setlength{\tabcolsep}{5pt}
\begin{tabular}{lrr}
Domain & Avg \# Articles  & Cohen's D \\ 
& Origin Topics  &   Effect Size\\ \midrule
theeconomiccollapseblog.com& 3.0930 & 1.3005 \\
thenationalpulse.com &1.725 &0.6290262\\
breaking911.com &  1.2&  0.492409\\
mercola.com & 2.32&  0.46424 \\
gellerreport.com &1.125 &  0.45163\\
Avg & & 0.03803611673394116 \\

\end{tabular}
\caption{\label{tab:real-originating} Most effective large popular websites in getting narratives spread onto other wesbites. Rank $<$ 1000 }  
\vspace{-5pt}
\end{table}

\begin{table}
\centering
%\fontsize{9pt}{10.5pt}
\scriptsize
\setlength{\tabcolsep}{5pt}
\begin{tabular}{lrr}
Domain & Avg \# Articles  & Cohen's D \\ 
& Origin Topics  &   Effect Size\\ \midrule
outragedpatriot.com&1.79  & 0.57261 \\
projectveritas.com & 2.38&0.54327\\
publicpolicypolling.com& 19.85 & 0.52887\\
analyzingamerica.org & 1.26&  0.50141420 \\
informationliberation.com & 10.193&  0.4661094\\
Avg & & 0.028418872007705046\\

\end{tabular}
\caption{\label{tab:real-originating} Most effective large popular websites in getting narratives spread onto other wesbites. Rank $<$ 1000 }  
\vspace{-5pt}
\end{table}


\begin{table}
\centering
%\fontsize{9pt}{10.5pt}
\scriptsize
\setlength{\tabcolsep}{5pt}
\begin{tabular}{lrr}
Domain & Avg \# Articles  & Cohen's D \\ 
& Origin Topics  &   Effect Size\\ \midrule
dutchsinse.com& 69.5 &  0.9969791 \\
thefreedomarticles.com & 1.0& 0.54211\\
covidvaccinevictims.com& 17.625 & 0.5021\\
thescoop.us&1.142 & 0.4697789\\
thetruthaboutvaccines.com & 0.972&  0.4544687\\
0.012382608153836506 & & \\
\end{tabular}
\caption{\label{tab:real-originating} Most effective large popular websites in getting narratives spread onto other wesbites. Rank $<$ 1000 }  
\vspace{-5pt}
\end{table}

\begin{table}
\centering
%\fontsize{9pt}{10.5pt}
\scriptsize
\setlength{\tabcolsep}{5pt}
\begin{tabular}{lrr}
Domain & Avg \# Articles  & Cohen's D \\ 
& Origin Topics  &   Effect Size\\ \midrule
other98.com& 1.6 &  0.832100 \\
stormcloudsgathering.com &46.33 & 0.812797\\
leftaction.com&10.2&0.665644\\
presscorp.org&3.82 &  0.62510\\
medicine.news &1.0 &   0.61713\\
Avg & & 0.00019066567191096325\\
\end{tabular}
\caption{\label{tab:real-originating} Most effective large popular websites in getting narratives spread onto other wesbites. Rank $<$ 1000 }  
\vspace{-5pt}
\end{table}

\begin{table}
\centering
%\fontsize{9pt}{10.5pt}
\scriptsize

\setlength{\tabcolsep}{5pt}
\begin{tabular}{lrr}
Domain & Avg \# Articles  & Cohen's D \\ 
& Origin Topics  &   Effect Size\\ \midrule
dailymail.co.uk & 11.25 &1.024\\%\hline 
express.co.uk & 9.107&0.6572\\%\hline 

Avg & 10.17 & 0.8407
\end{tabular}
\caption{\label{tab:real-originating} Most effective large popular websites in getting narratives spread onto other wesbites. Rank $<$ 1000 }  
\vspace{-5pt}
\end{table}


\begin{table}
\centering
%\fontsize{9pt}{10.5pt}
\scriptsize

\setlength{\tabcolsep}{5pt}
\begin{tabular}{lrr}
Domain & Avg \# External Articles  & Cohen's D \\ 
& per Origin Topic  &   Effect Size\\ \midrule
mirror.co.uk &6.842&0.0.85109\\
rt.com & 15.06& 0.81317 \\
zerohedge.com &18.32 &  0.8018 \\
nypost.com  & 11.105& 0.792\\
breitbart.com & 12.1572& 0.74465 \\
Avg & 12.697 &0.8007\\
\end{tabular}
\caption{\label{tab:real-originating} Most effective large popular websites in getting narratives spread onto other wesbites. Rank $<$ 1000 }  
\vspace{-5pt}
\end{table}

\begin{table}
\centering
%\fontsize{9pt}{10.5pt}
\scriptsize

\setlength{\tabcolsep}{5pt}
\begin{tabular}{lrr}
Domain & Avg \# Articles  & Cohen's D \\ 
& Origin Topics  &   Effect Size\\ \midrule
dailystar.co.uk & 10.3668 &  1.553 \\
thegatewaypundit.com &14.876 &0.7669\\
newsmax.com &11.9859 &0.763\\
bleacherreport.com &4.1480& 00.747 \\
rawstory.com &11.2062 & : 0.5669\\
Avg & 7.607&0.6605\\


\end{tabular}
\caption{\label{tab:real-originating} Most effective large popular websites in getting narratives spread onto other wesbites. Rank $<$ 1000 }  
\vspace{-5pt}
\end{table}






\begin{table}
\centering
%\fontsize{9pt}{10.5pt}
\scriptsize

\setlength{\tabcolsep}{5pt}
\begin{tabular}{lrr}
Domain & Avg \# Articles  & Cohen's D \\ 
& Origin Topics  &   Effect Size\\ \midrule
newsbreak.com& 15.8646 &  2.8113 \\
westernjournal.com & 17.4349&  1.2355\\
thecut.com&  31.866&  1.227639 \\
dailycaller.com &14.5266 & 1.21777\\
theblaze.com& 15.6241&   1.203938 \\
Avg &9.82 &0.792 \\

\end{tabular}
\caption{\label{tab:real-originating} Most effective large popular websites in getting narratives spread onto other wesbites. Rank $<$ 1000 }  
\vspace{-5pt}
\end{table}


\begin{table}
\centering
%\fontsize{9pt}{10.5pt}
\scriptsize
\setlength{\tabcolsep}{5pt}
\begin{tabular}{lrr}
Domain & Avg \# Articles  & Cohen's D \\ 
& Origin Topics  &   Effect Size\\ \midrule
theconservativetreehouse.com& 22.287 &1.38547 \\
oann.com & 17.435&1.2571\\
resistthemainstream.org & 12.567&  1.2492 \\
thefederalist.com &29.76&    1.224 \\
dennismichaellynch.com &12.893 &1.18779 \\
Avg & 10.21& 0.7725396 \\

\end{tabular}
\caption{\label{tab:real-originating} Most effective large popular websites in getting narratives spread onto other wesbites. Rank $<$ 1000 }  
\vspace{-5pt}
\end{table}

\begin{table}
\centering
%\fontsize{9pt}{10.5pt}
\scriptsize
\setlength{\tabcolsep}{5pt}
\begin{tabular}{lrr}
Domain & Avg \# Articles  & Cohen's D \\ 
& Origin Topics  &   Effect Size\\ \midrule
tbdailynews.com &12.1974& 3.425989\\
thepatriotjournal.com& 22.1978 &  2.34418\\
therightscoop.comm & 15.951&  1.832 \\
weaselzippers.us & 5.1986&  1.4607 \\
headlineusa.com & 33.2&  1.35960\\
Avg &12.522 &0.7900 \\

\end{tabular}
\caption{\label{tab:real-originating} Most effective large popular websites in getting narratives spread onto other wesbites. Rank $<$ 1000 }  
\vspace{-5pt}
\end{table}



\begin{table}
\centering
%\fontsize{9pt}{10.5pt}
\scriptsize
\setlength{\tabcolsep}{5pt}
\begin{tabular}{lrr}
Domain & Avg \# Articles  & Cohen's D \\ 
& Origin Topics  &   Effect Size\\ \midrule
theconservativebrief.com& 5.8638 & 1.97176 \\
shtfplan.com &5.7716 &1.81145\\
uncoverdc.com & 23.4861 &   1.797\\
yournews.com &8.6279 &  1.5890 \\
nationalfile.com& 19.4762&  1.51334\\
Avg & & 0.8133\\

\end{tabular}
\caption{\label{tab:real-originating} Most effective large popular websites in getting narratives spread onto other wesbites. Rank $<$ 1000 }  
\vspace{-5pt}
\end{table}

\begin{table}
\centering
%\fontsize{9pt}{10.5pt}
\scriptsize
\setlength{\tabcolsep}{5pt}
\begin{tabular}{lrr}
Domain & Avg \# Articles  & Cohen's D \\ 
& Origin Topics  &   Effect Size\\ \midrule
english.cctv.com&7.697  & 2.328 \\
conservativeangle.com &9.6989 &2.1214\\
en-volve.com& 6.1978 & 1.8677\\
genzconservative.com & 52.199&  1.73170 \\
conservativefreepress.com &18.20 &  .63033\\
Avg &11.71 & 0.8109\\

\end{tabular}
\caption{\label{tab:real-originating} Most effective large popular websites in getting narratives spread onto other wesbites. Rank $<$ 1000 }  
\vspace{-5pt}
\end{table}


\begin{table}
\centering
%\fontsize{9pt}{10.5pt}
\scriptsize
\setlength{\tabcolsep}{5pt}
\begin{tabular}{lrr}
Domain & Avg \# Articles  & Cohen's D \\ 
& Origin Topics  &   Effect Size\\ \midrule
christianaction.org& 34.698 & 1.759 \\
libertyunyielding.com& 21.70& 1.6203\\
thejeffreylord.com& 19.197 &  1.342\\
lancastercourier.com&6.1987 & 1.274628\\
marzlovesfreedom.com& 10.197&  1.2729\\
Avg & 8.250 &0.77559  \\
\end{tabular}
\caption{\label{tab:real-originating} Most effective large popular websites in getting narratives spread onto other wesbites. Rank $<$ 1000 }  
\vspace{-5pt}
\end{table}

\begin{table}
\centering
%\fontsize{9pt}{10.5pt}
\scriptsize
\setlength{\tabcolsep}{5pt}
\begin{tabular}{lrr}
Domain & Avg \# Articles  & Cohen's D \\ 
& Origin Topics  &   Effect Size\\ \midrule
yc.news&  18.0339&  1.8548 \\
presscorp.org &20.6985 & 1.61182\\
climate.news& 4.9470 &1.57977\\
freetelegraph.com& 10.1975&  1.34276\\
thefreedomtimes.com& 19.541&    1.28307\\
Avg &11.130 & 0.7930\\
\end{tabular}
\caption{\label{tab:real-originating} Most effective large popular websites in getting narratives spread onto other wesbites. Rank $<$ 1000 }  
\vspace{-5pt}
\end{table}


\begin{figure}
\begin{subfigure}{.45\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/communities.png}
\end{subfigure}%

\label{fig:website-domains-over-time}
\caption{Communities of semantically similar websites. Node size is determined by the PageRank metric. 
}
\end{figure}


Topic 7 &putin,russia,president,west,vladmir &\tiny {Since Vladimir Putin's official return to power in 2012} & \tiny{Putin today has stepped } \\
& &  \tiny {the Russian president seems to have set his mind} & \tiny{into the role of the ``Great} \\
& &  \tiny {on teaching the rest of the world} & \tiny{Russian executioner'' of the Ukrainian people to } \\
& &  \tiny {a few simple lessons.} & \tiny{remember Lenin s words, reigniting} \\
& &  \tiny {First, that he shall not be underestimated} & \tiny{the old Tzarist supremacist impulses.} \\
\midrule

Topic 8 &homicide,crime,murder,violent,robery & \tiny {As I noted in a January review of American cities with} & \tiny{Violent crime is on the rise across the country} \\
& &  \tiny {huge crime spikes, local media outlet} & \tiny{especially in big blue cities.} \\
& &  \tiny {KTTV Fox 11 reported in 2021 an 11.8 increase in homicides} & \tiny{Some New Yorkers are scared to ride the subway} \\
& &  \tiny {while violent crime increased 3.9} & \tiny{following a violent shooting in Brooklyn last month.} \\ \midrule

Topic 9 &sanction,impose,russia,putin,moscow & \tiny{The US and its allies in Europe and beyond} & \tiny{Since the start of Russia’s military campaign}\\
& &  \tiny{have imposed an unprecedented number of sanctions} & \tiny{in Ukraine on February 24, the US, UK, Canada, Australia, EU members}\\
& &  \tiny{against Russia over its military offensive.} & \tiny{Japan, and few others have imposed several rounds}\\
& &  \tiny{} & \tiny{of unprecedented sanctions on Russia.}\\ \midrule

Topic 10 &clinton,trump,collusion,server,campaign & \tiny{The Trump launched Durham probe into the origins of the } & \tiny{Today's corrupt DOJ and FBI worked with the Hillary Clinton} \\
& &  \tiny{Russian collusion scandal recently revealed} & \tiny{ campaign to conjure up a lie that candidate} \\
& &  \tiny{that not only did the bogus collusion narrative} & \tiny{and then President Trump was involved } \\
& &  \tiny{originate with the Hillary Clinton campaign} & \tiny{with Putin and Russia in some kind} \\
& &  \tiny{but that she personally approved} & \tiny{ of clandestine partnership.} \\
& &  \tiny{leaking to the media a phony story claiming the Trump } & \tiny{There was no evidence of this. They made it up.} \\
& &  \tiny{ campaign had been in contact with Russia s Alfa Bank. } & \tiny{} \\


\begin{table*}
\centering
\scriptsize
%\fontsize{8.5pt}{10pt}
\selectfont
\begin{tabular}{l|r|l|r|l|r}
Top Topics on 8kun & \# Comm. & Top Topics on 4chan & \# Comm. & Top Topics on Reddit &  \# Comm. \\ \toprule
disinformation,propaganda,conspiracy,expose,fake &1,285 & jew,judaism,zionist,israel,liberal & 4,001 & beautiful,furry,sheila,adorable,wow &78,194\\
 research,shill,comms,potus,batten&1,193 & jew,goy,white,zionist,supremacist &3,216 & tip,restaurant,customer,server,gratuity&60,994 \\
 qanon,conspiracy,theory,pedophile,cabal &1,157 & flat,earth,globe,spherical,theory &1,756 &  onlyfans,creator,porn,subscription,platform &55,677 \\
  rally,donald,trump,45th,arizona & 858& white,race,racism,caucasian,whiteness &1,576 & foot,toe,tally,heel,fetish & 45,381 \\
  fbi,investigation,comedy,doj,trump  &838 & ukraine,russia,nato,conflict,invasion &1,218& gentleman,way,man,foolish,agree & 44,078 \\ 
\end{tabular}
\caption{\label{tab:social-media-posts} Top narratives from our set of unreliable websites present on different social media platforms} 
\end{table*}

\begin{table*}
\centering
\scriptsize
%\fontsize{8.5pt}{10pt}
\selectfont
\begin{tabular}{l|l}
Domain & Most Similar Subreddits (by JS-Divergence) \\ \toprule
rt.com & credibledefense (0.277)  worldnews (0.288), endlesswar (0.295), ukrainianconflict (0.304), chomsky (0.305) \\
zerohedge.com & wayofthebern (0.278), atayls (0.290), thewallstreet (0.292), vitards (0.292), prepperintel (0.292) \\

breitbart.com & conservative (0.300),  moderatepolitics (0.317)  conservatives (0.317), enough\_sanders\_spam (0.320), republican (0.320) \\
americanthinker.com & conservative (0.212), walkaway (0.223),  timpool (0.239), louderwithcrowder (0.239), wayofthebern (0.240) \\
theepochtimes.com & wayofthebern (0.291),prepperintel (0.305),  canada\_sub (0.307),conservativekiwi (0.308),walkaway (0.309),\\

\end{tabular}
\caption{\label{tab:social-media-posts} Most similar subreddits--according to topic distribution (JS-Divergence)-- to a select set of websites from our dataset.} 
\end{table*}

\begin{table*}
\centering
\scriptsize
%\fontsize{8.5pt}{10pt}
\selectfont
\begin{tabular}{l|l|r|r|l}
Plaform & \# of Posts & \# correponding narrative & JS-Similarity to All Unreliable Websites & Most similar Unreliable Websites  \\\toprule
8kun.top & 1,207,521 & 399,850 (33.1\%) & 0.2016 &beforeitsnews.com,radiopatriot.net,ussanews.com \\
4chan.org & 2,487,527 & 438,047 (17.10\%) & 0.2479 & unz.com,abovetopsecret.com, thetruthseeker.co.uk\\
reddit.com & 238,515,614 &40,689,998 (16.45\%)& 0.3111 & abovetopsecret.com,herbeauty.co,cochrane.org\\
\end{tabular}
\caption{\label{tab:social-media-posts} Our dataset of social media posts and their relationship to the narratives promoted by our set of unreliable websites.} 
\end{table*}


\section{Fact-Checking at Different Thresholds\label{sec:fact-thresh}}
\begin{table}[h]
\centering
%\setlength\tabcolsep{4pt}
\scriptsize
\begin{tabular}{l|lllll}
\toprule
& \# Narratives & Avg.  &Avg.  \\ 
&{Fact }   & {Days to }  &{Days from }  &{\# 0-Day }  \\ 
&{Checked}   & {Fact-Check} &{Narrative Peak } & {Fact-Checks} \\ \toprule
Politifact & 865 &130.8  & 12.6 & 2 \\
Reuters & 1339 & 134.1 &5.4 & 19  \\
AP News & 124 & 109.1 & -10.6 &1 \\
\bottomrule
\end{tabular}
\caption{\label{tab:fact-check} Efficacy of Different Fact-checking websites at threshold of 0.80.} 
\vspace{-15pt}
\end{table}



\begin{table}[h]
\centering
%\setlength\tabcolsep{4pt}
\scriptsize
\begin{tabular}{l|lllll}
\toprule
& \# Narratives & Avg.  &Avg.  \\ 
&{Fact }   & {Days to }  &{Days from }  &{\# 0-Day }  \\ 
&{Checked}   & {Fact-Check} &{Narrative Peak } & {Fact-Checks} \\ \toprule
Politifact & 2917 &124.9  & 16.4 & 2 \\
Reuters & 3824 & 123.4 &8.3 & 34  \\
AP News & 386 & 110.7 & -4.7 &1 \\
\bottomrule
\end{tabular}
\caption{\label{tab:fact-check} Efficacy of Different Fact-checking websites at threshold of 0.70.} 
\vspace{-15pt}
\end{table}


\begin{table}[h]
\centering
%\setlength\tabcolsep{4pt}
\scriptsize
\begin{tabular}{l|lllll}
\toprule
& \# Narratives & Avg.  &Avg.  \\ 
&{Fact }   & {Days to }  &{Days from }  &{\# 0-Day }  \\ 
&{Checked}   & {Fact-Check} &{Narrative Peak } & {Fact-Checks} \\ \midrule
Politifact & 4354 &121.1  & 16.1 & 2 \\
Reuters & 5323 & 120.8 &11.0 & 42  \\
AP News & 511 & 113.9 & -2.0 &1 \\
\bottomrule
\end{tabular}
\caption{\label{tab:fact-check} Efficacy of Different Fact-checking websites at threshold of 0.65.} 
\end{table}

\begin{table}
\centering
\scriptsize
%\setlength\tabcolsep{4pt}
\begin{tabular}{l|lll}
\toprule
Threshold & Precision & Estimated Recall  & F1-Score  \\ \midrule
0.60 & 66.5\% & --&-- \\
0.65 & 70.4\% &\textbf{89.8\%} & 0.789  \\
0.70 & 82.9\% & 79.8\% &\textbf{0.813}\\
0.75 &93.8\% & 56.9\% &0.708\\
0.80 & \textbf{97.6\%} & 30.1\%&0.460 \\
\bottomrule
\end{tabular}
\caption{\label{tab:fact-check} Precision, Recall, and F-1 Scores of fact-checks assigned to different narrative clusters.} 
\vspace{-5pt}
\end{table}



\begin{table}
\centering
\setlength\tabcolsep{4pt}
\scriptsize
\begin{tabular}{llr}
\toprule
Website 1 & Website 2 & JS-Divergence \\ \midrule
peternavarro.comm & somebitchtoldme.com & 0.0322 \\
israeli-connections-to-911.com & pl911truth.com &  0.0344\\
realjewnews.com &secondamendmentdaily.com&  0.0344 \\
1000covidstories.com& virus-hoax.com& 0.0344\\
911truthactivism.blogspot.com & iran911case.com  &  0.0350\\ \midrule
express.co.uk & gotquestions.org &   0.7491\\

bleacherreport.com & thetrumpet.com &   0.7424\\

prevention.com& southfront.org &   0.7242 \\
childrenshealthdefense.org & tass.com & 0.7170 \\
hotair.com & prevention.com  &0.7067\\
\bottomrule
\end{tabular}
\caption{\label{tab:js-sim} Examples of websites with the greatest (JS-D=0) and least (JS-D=1) similarity to each other using JS-Divergence of the distribution of the narratives/stories each website addressed.}
\vspace{-10pt}
\end{table}


6 & ukraine, nato, putin, russia, war & 6,812 & 417 & sott.net (276), theautomaticearth.com (196), veteranstoday.com (194) & To call the US and Western stance on Russian involvement in Ukraine 'hypocritical' really doesn't accurately describe the egregious mendacity exhibited by Western psychopaths in power. The current war between Russia and Ukraine is really a proxy war\\ \midrule
 7&  missile, donetsk, ukraine, artillery, strike & 6,758 & 321& tass.com (597), southfront.org (476), dailymail.co.uk (415) & Russian military jets are flying over Ukrainian airspace, targeting the country s military infrastructure. missiles are pounding different cities from capital Kiev to Kharkiv. Russia carried out strikes on military infrastructure sites in western Ukraine using long-range precision weapons. \\ \midrule
 8 & gallon, average, aaa, gasoline, price & 5,179 & 356 & theepochtimes.com (243), nypost.com (207), shorenewsnetwork.com (195) & he national average price of a gallon of gasoline was 4.17 as of Tuesday morning, according to AAA data. The latest numbers shatter the previous record of 4.11 established in July 2008. Gas prices jumped 25 cents from last week \\ \midrule
 9 & fed, hike, inflation, tighten, monetary & 5,162 & 253 & shorenewsnetwork.com (1407), theepochtimes.com (490), zerohedge.com (335) & Traders hope signs economic activity is slowing and inflation pressures easing might prompt the Fed to ease off its plans. Fed officials including chair Jerome Powell have warned rates might need to stay high for an extended period to extinguish inflation.\\ \midrule
 10&  roe, abort, wade, overturn, 1973 & 4,884 & 403& shorenewsnetwork.com (175), theepochtimes.com (170), dailymail.co.uk (148) & Friday overturned Roe v. Wade, effectively ending recognition of a constitutional right to abortion. This gives individual states the power to allow, limit, or ban the practice altogether. Nearly half of the states already have laws that ban abortion.\\

==> originEcho.tex <==








==> preliminaries.tex <==
\section{Preliminaries}
\todo{You'll probably see from the comments, I suggested that you take the content in this section and split it into a few others. I don't think I've seen a Preliminaries section like this in an Oakland paper and there are better homes for the content in the typical paper structure (e.g., background, dataset)}

\todo{This paragraph is good introduction material. We won't need to repeat it again here (and shouldn't given page limits)}
  In this section, we specify the definitions, requirements, and the dataset that this system utilizes. 


\TODO{it'd be good to define some adjective that we use throughout the paper to describe the set of ``unreliable'' sites we use. Otherwise it's going to get wordy. I think ``unreliable'' is a good term if we define it once at the start}






